Edited Media Understanding Frames: Reasoning About the Intent and Implications of Visual Misinformation

Multimodal disinformation, from 'deepfakes' to simple edits that deceive, is an important societal problem. Yet at the same time, the vast majority of media edits are harmless -- such as a filtered vacation photo. The difference between this example, and harmful edits that spread disinformation, is one of intent. Recognizing and describing this intent is a major challenge for today's AI systems. We present the task of Edited Media Understanding, requiring models to answer open-ended questions that capture the intent and implications of an image edit. We introduce a dataset for our task, EMU, with 48k question-answer pairs written in rich natural language. We evaluate a wide variety of vision-and-language models for our task, and introduce a new model PELICAN, which builds upon recent progress in pretrained multimodal representations. Our model obtains promising results on our dataset, with humans rating its answers as accurate 40.35% of the time. At the same time, there is still much work to be done -- humans prefer human-annotated captions 93.56% of the time -- and we provide analysis that highlights areas for further progress.

==> tables/results_dims.tex <==
\definecolor{lightgray}{rgb}{0.99, 0.99, 0.99}
\newcolumntype{g}{>{\columncolor{lightgray}}c}
\begin{table}[]
\centering
\begin{tabular}{l||c||c}
\multicolumn{1}{c}{} & \multicolumn{1}{g}{{\smaller Automatic Eval}} & \multicolumn{1}{g}{{\smaller Human Eval}}\\
Question \dimension & \thead{Accuracy $\uparrow$} & \thead{Accurate \% $\uparrow$} \\ \toprule
\textsc{Intent} & 54.03 & 62.68 \\
\textsc{Implication} & 53.84 & 45.37 \\
\textsc{Disinformation} & 57.64 & 52.65 \\
\textsc{\subjectX \space implicate} & 55.14 & 90.46 \\
\textsc{\subjectX \space emotion} & 55.64 & 66.14 \\
\end{tabular}
\caption{Results for generations produced by \modelname \space per \dimension. \modelname \space is able to reason accurately across a variety of \dimensions \space -- yet, difficulty of each \dimension \space varies drastically. \antoine{be a bit wary here. you also show that your auto eval correlates poorly with your human eval. Might be good to remind the reader if they're testing different dimensions of the problem. Also unless your label distribution is balances for the automatical evaluation, you might want to report precision/recall too.}}
\label{fig:results_dim}
\end{table}


